Point Primitive Transformer for Long-Term 4D Point Cloud Video Understanding

This paper proposes a 4D backbone for long-term point cloud video understanding. A typical way to capture spatial-temporal context is using 4Dconv or transformer without hierarchy. However, those methods are neither effective nor efficient enough due to camera motion, scene changes, sampling patterns, and the complexity of 4D data. To address those issues, we leverage the primitive plane as a mid-level representation to capture the long-term spatial-temporal context in 4D point cloud videos and propose a novel hierarchical backbone named Point Primitive Transformer(PPTr), which is mainly composed of intra-primitive point transformers and primitive transformers. Extensive experiments show that PPTr outperforms the previous state of the arts on different tasks.

==> [ECCV2022] 4DPrimitiveTransformer/tex/abstract.tex <==
This paper proposes a 4D backbone for long-term point cloud video understanding. A typical way to capture spatial-temporal context is using 4Dconv or transformer without hierarchy. However, those methods are neither effective nor efficient enough due to camera motion, scene changes, sampling patterns, and complexity of 4D data. To address those issues, we leverage the primitive plane as mid-level representation to capture the long-term spatial-temporal context in 4D point cloud videos, and propose a novel hierarchical backbone named Point Primitive Transformer(PPTr), which is mainly composed of intra-primitive point transformers and primitive transformers. Extensive experiments show that PPTr outperforms the previous state of the arts on different tasks.

==> [ECCV2022] 4DPrimitiveTransformer/tex/conclusion.tex <==
This paper proposes a 4D backbone for long-term point cloud video understanding. The key idea is to leverage the primitive plane to capture the long-term spatial-temporal context in 4D point cloud videos. Results of experiments showing ablations and state-of-the-art performance on a wide range of 4D tasks including MSR-Action3D action recognition task, 4D semantic segmentation on sythia4D and on HOI4D. This result is very encouraging and suggests future work to explore more possible backbone designs for 4D point cloud understanding. 

==> [ECCV2022] 4DPrimitiveTransformer/tex/exp.tex <==
\subsection{4D Semantic Segmentation}
\textbf{Setup.} Temporal information can help understand the dynamic objects in the scene, and improve segmentation accuracy and robustness to noise. Due to memory constraints, existing methods only process point cloud videos with a length of 3. Our method can consider a longer temporal range and achieve a more efficient integration of spatio-temporal information. In this task, we fit the scene point cloud into 200 primitives. 
% We sort all the points according to the primitive, and divide them into 200 sub-point sets with the same number of points.
We use mean IoU(mIoU) \%  as the evaluation metric.

\subsubsection{4D Semantic Segmentation on Synthia 4D dataset.}
\textbf{Setup.} Synthia 4D~\cite{synthia} is a synthetic dataset for outdoor autonomous driving. It creates 3D videos with the Synthia dataset, which consists of six videos of driving scenarios in which objects and cameras are moving. We use the same training/validation/test split as previous work, with 19,888/815/1,886 frames, respectively. 


% \resizebox{10mm}{5mm}{
% \newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}} 
% \begin{table}
% \setlength{\tabcolsep}{0.2mm}
% \tiny{
% \begin{center}
% \caption{Evaluation for semantic segmentation on Synthia 4D dataset~\cite{synthia}}
% \label{table:synthia4d}
% \begin{tabular}{l|c|c|cccccccccccc|c}
% \hline\noalign{\smallskip}
% Method & Frames & \tabincell{c}{-} & Bldn& Road& Sdwlk & Fence& Vegittn & Pole & Car & T.Sign & Pedstrn & Bicycl & Lane & T.Light& mIoU\\
% \noalign{\smallskip}
% \hline
% \noalign{\smallskip}
% 3D MinkNet14~\cite{minkowski}& 1& - & 89.39& 97.68&69.43 &86.52 &98.11 &97.26 &93.50 &79.45 &92.27 & 0.00 & 44.61 & 66.69 & 76.24\\
% 4D MinkNet14~\cite{minkowski}& 3& - & 90.13& 98.26& 73.47& 87.19& 99.10& 97.50& 94.01& 79.04& \textbf{92.62}& 0.00 & 50.01 & 68.14 & 77.24\\
% \hline
% \noalign{\smallskip}
% PointNet++~\cite{pointnet2} & 1& - & 96.88 &  97.72 & 86.20 & 92.75 & 97.12 & 97.09 & 90.85 & 66.87 & 78.64 & 0.00 & 72.93 & 75.17 & 79.35 \\
% MeteorNet-m~\cite{meteornet} & 2& - & \textbf{98.22} & 97.79 & 90.98 & 93.18 & 98.31 & 97.45 & 94.30 & 76.35  & 81.05 & 0.00 & 74.09 & 75.92& 81.47 \\
% MeteorNet-l~\cite{meteornet} & 3& - & 98.10 & 97.72  & 88.65 & 94.00 & 97.98 & 97.65 & 93.83 & \textbf{84.07}  & 80.90  &0.00 & 71.14 & 77.60 & 81.80\\
% \noalign{\smallskip}
% \hline
% \noalign{\smallskip}
% P4Transformer~\cite{p4transformer} & 1& - & 96.76 & 98.23 & 92.11 & 95.23 & 98.62 & 97.77 & 95.46 & 80.75 & 85.48 & 0.00 & 74.28 & 74.22 & 82.41\\
% P4Transformer~\cite{p4transformer} & 3& - & 96.73 & 98.35 & 94.03 & 95.23 & 98.28 & 98.01 & 95.60 & 81.54 & 85.18 & 0.00 & 75.95 & \textbf{79.07} & 83.16 \\
% \noalign{\smallskip}
% \hline
% \noalign{\smallskip}
% \tiny{PPTr(ours)} & 1& 0 &97.14 &98.42 &94.12 & 97.00&99.59 & 97.86 & 98.54 & 79.68 & 89.20 & 0.00 & 77.26 & 77.42 & 83.85\\
% \tiny{PPTr(ours)} & 1& 30 &98.01 &\textbf{98.63} &\textbf{95.26} &\textbf{97.03} & \textbf{99.70}&\textbf{97.95} &\textbf{98.76} & 81.99&91.20&0.00&\textbf{78.29}&77.09&\textbf{84.49}\\
% % \tiny{4DHPT(ours)} & 3& 0 & & & & & & & & &\\
% % \tiny{4DHPT(ours)} & 3& 0 & & & & & & & & &\\
% \noalign{\smallskip}
% \hline
% \end{tabular}
% \end{center}
% }
% \end{table}
% }

\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}} 
\begin{table}
\setlength{\tabcolsep}{0.2mm}
\tiny{
\begin{center}
\caption{Evaluation for semantic segmentation on Synthia 4D dataset~\cite{synthia}}
\label{table:synthia4d}
\begin{tabular}{l|c|cccccccccccc|c}
\hline\noalign{\smallskip}
Method & Frames & Bldn& Road& Sdwlk & Fence& Vegittn & Pole & Car & T.Sign & Pedstrn & Bicycl & Lane & T.Light& mIoU\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
3D MinkNet14~\cite{minkowski}&1 & 89.39& 97.68&69.43 &86.52 &98.11 &97.26 &93.50 &79.45 &92.27 & 0.00 & 44.61 & 66.69 & 76.24\\
4D MinkNet14~\cite{minkowski}& 3 & 90.13& 98.26& 73.47& 87.19& 99.10& 97.50& 94.01& 79.04& \textbf{92.62}& 0.00 & 50.01 & 68.14 & 77.24\\
\hline
\noalign{\smallskip}
PointNet++~\cite{pointnet2} & 1& 96.88 &  97.72 & 86.20 & 92.75 & 97.12 & 97.09 & 90.85 & 66.87 & 78.64 & 0.00 & 72.93 & 75.17 & 79.35 \\
MeteorNet-m~\cite{meteornet} & 2 & \textbf{98.22} & 97.79 & 90.98 & 93.18 & 98.31 & 97.45 & 94.30 & 76.35  & 81.05 & 0.00 & 74.09 & 75.92& 81.47 \\
MeteorNet-l~\cite{meteornet} & 3 & 98.10 & 97.72  & 88.65 & 94.00 & 97.98 & 97.65 & 93.83 & \textbf{84.07}  & 80.90  &0.00 & 71.14 & 77.60 & 81.80\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
P4Transformer~\cite{p4transformer} & 1 & 96.76 & 98.23 & 92.11 & 95.23 & 98.62 & 97.77 & 95.46 & 80.75 & 85.48 & 0.00 & 74.28 & 74.22 & 82.41\\
P4Transformer~\cite{p4transformer} & 3 & 96.73 & 98.35 & 94.03 & 95.23 & 98.28 & 98.01 & 95.60 & 81.54 & 85.18 & 0.00 & 75.95 & \textbf{79.07} & 83.16 \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
\tiny{PPTr(ours)} & 1 &97.14 &98.42 &94.12 & 97.00&99.59 & 97.86 & 98.54 & 79.68 & 89.20 & 0.00 & 77.26 & 77.42 & 83.85\\
\tiny{PPTr(ours)} & 30 &98.01 &\textbf{98.63} &\textbf{95.26} &\textbf{97.03} & \textbf{99.70}&\textbf{97.95} &\textbf{98.76} & 81.99&91.20&0.00&\textbf{78.29}&77.09&\textbf{84.49}\\
% \tiny{4DHPT(ours)} & 3& 0 & & & & & & & & &\\
% \tiny{4DHPT(ours)} & 3& 0 & & & & & & & & &\\
\noalign{\smallskip}
\hline
\end{tabular}
\end{center}
}
\end{table}

\textbf{Result.} Table~\ref{table:synthia4d} shows our method outperforms the state-of-the-art methods. Our PPTr with 1 frame can achieve $0.69\%$ improvement over the P4Transformer with 3 frames, which demonstrates the effectiveness of the hierarchical structure. When using the memory pool to integrate temporal information from 30 frames, we can achieve $1.33\%$ improvement over previous state-of-the-art methods. It is worth mentioning that our method is the first to integrate point clouds of 30 frames, which is 10 times that of previous methods. And we also demonstrate that longer point cloud sequences are valuable for 4D semantic segmentation.

% achieves $1.33\%$ improvement over the P4Transformer.
\subsubsection{4D Semantic Segmentation on HOI4D.}
\textbf{Setup.} In order to further verify the effectiveness of our method, we select the HOI4D dataset for experiments, which is a large-scale 4D egocentric dataset to catalyze the research of category-level human-object interaction. It provides frame-wise annotations for 4D point cloud semantic segmentation. Since the dataset has not been released yet, we sent an email to the author team to request 1000 sequences, which includes 30k frames of the point cloud. The train/test split is the same as HOI4D.


% \resizebox{10mm}{5mm}{
% \newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}} 
% \begin{table}
% \setlength{\tabcolsep}{0.15mm}
% \scriptsize{
% \begin{center}
% \caption{Evaluation for semantic segmentation on HOI4D dataset~\cite{liu2022hoi4d}}
% \label{table:hoi4d}
% \begin{tabular}{l|c|c|ccccccccc|c}
% \hline\noalign{\smallskip}
% Method & Frames & \tabincell{c}{Pool\\Size} & Table &Ground  & Metope &Locker & Pliers  &Laptop &\tabincell{c}{Safe\\Deposit} &Pillow &\tabincell{c}{Hand \\and Arm}& mIoU\\
% \noalign{\smallskip}
% \hline
% \noalign{\smallskip}
% % PointNet++& 1& - & & & & & & & & &\\
% \tiny{PSTNet~\cite{pstnet}} & 3& - &	57.45 &	63.38 &	83.80 &	44.69 &	13.71 &	35.03 &	51.55 &	76.30 &	40.39 &51.81 \\
% \tiny{P4Transformer~\cite{p4transformer}} & 1& - & 60.84 &  71.98   &	86.69 &	53.89 &	34.00 &	65.89 &	55.87 &	52.19 &	55.10 & 59.61 \\
% \tiny{P4Transformer~\cite{p4transformer}} & 3& - & 63.58 &	66.60 &	87.17 &	58.39 &	32.29 &	72.03 &	65.87 &	57.41 &	54.36 & 61.97 \\
% \noalign{\smallskip}
% \hline
% \noalign{\smallskip}
% \tiny{PPTr(ours)} & 1& 0 &	67.73 &	74.08 &	90.27 &	\textbf{61.50} &	39.37 &	66.05 &	71.20 &\textbf{85.78} &	53.77 & 67.75 	 \\
% \tiny{PPTr(ours)} & 1& 30 & \textbf{69.18} &	\textbf{78.84} &\textbf{91.08}	 &	61.30 &	\textbf{39.41} &	\textbf{74.18} &	\textbf{72.00} &	66.80 &	\textbf{61.42} & \textbf{68.25}\\
% % \scriptsize{4DHPT(ours)} & 3& 0 & & & & & & & & &\\
% % \scriptsize{4DHPT(ours)} & 3& 10 & & & & & & & & &\\
% \noalign{\smallskip}
% \hline
% \end{tabular}
% \end{center}
% }
% \end{table}
% }

\begin{table}
\setlength{\tabcolsep}{0.15mm}
\scriptsize{
\begin{center}
\caption{Evaluation for semantic segmentation on HOI4D dataset~\cite{liu2022hoi4d}}
\label{table:hoi4d}
\begin{tabular}{l|c|ccccccccc|c}
\hline\noalign{\smallskip}
Method & Frames  & Table &Ground  & Metope &Locker & Pliers  &Laptop &\tabincell{c}{Safe\\Deposit} &Pillow &\tabincell{c}{Hand \\and Arm}& mIoU\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
% PointNet++& 1& - & & & & & & & & &\\
\tiny{PSTNet~\cite{pstnet}} & 3&	57.45 &	63.38 &	83.80 &	44.69 &	13.71 &	35.03 &	51.55 &	76.30 &	40.39 &51.81 \\
\tiny{P4Transformer~\cite{p4transformer}} & 1 & 60.84 &  71.98   &	86.69 &	53.89 &	34.00 &	65.89 &	55.87 &	52.19 &	55.10 & 59.61 \\
\tiny{P4Transformer~\cite{p4transformer}} & 3 & 63.58 &	66.60 &	87.17 &	58.39 &	32.29 &	72.03 &	65.87 &	57.41 &	54.36 & 61.97 \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
\tiny{PPTr(ours)} & 1&	67.49 &	74.92 &	87.92 &	\textbf{62.12} &	40.06 &	69.00 &	71.39 & 77.18 &	62.50 & 68.07 	 \\
\tiny{PPTr(ours)} & 3& 66.78 &	72.76 &88.21	 &	60.83 &	\textbf{41.22} &	72.04 &	73.10 &	80.64 &	61.27 & 68.54\\
\tiny{PPTr(ours)} & 30& \textbf{67.76} &	\textbf{79.55} &\textbf{90.67}	 &	59.43 &	39.43 &	\textbf{72.67} &	\textbf{73.29} &	\textbf{84.13} & \textbf{64.26} & \textbf{70.13}\\
% \tiny{PPTr(ours)} & 1&	67.73 &	74.08 &	90.27 &	\textbf{61.50} &	39.37 &	66.05 &	71.20 &\textbf{85.78} &	53.77 & 67.75 	 \\
% \tiny{PPTr(ours)} & 30& \textbf{69.18} &	\textbf{78.84} &\textbf{91.08}	 &	61.30 &	\textbf{39.41} &	\textbf{74.18} &	\textbf{72.00} &	66.80 &	\textbf{61.42} & \textbf{68.25}\\
% \scriptsize{4DHPT(ours)} & 3& 0 & & & & & & & & &\\
% \scriptsize{4DHPT(ours)} & 3& 10 & & & & & & & & &\\
\noalign{\smallskip}
\hline
\end{tabular}
\end{center}
}
\end{table}


% \subsubsection{Visualization}

\textbf{Result.} As shown in Table~\ref{table:hoi4d}, our method outperforms previous methods on this more challenging dataset. Compared with P4transformer, the mIoU goes up from $59.61\%$ to $68.07\%$ and $61.97\%$ to $68.54\%$ in the case of single frame and 3 frames respectively, demonstrating the effectiveness of the hierarchical design again. Due to the limitation of computational resources, P4Transformer can use up to 3 frames, but our method can integrate 30 frames of spatio-temporal information. The improvement from $61.97\%$ to $70.13 \%$ further confirms that with our proposed primitive memory pool, we can better leverage the long-term temporal information to boost the 4D segmentation performance. 

\subsection{3D Action Recognition on MAR-Action3D}
\textbf{Setup.} To demonstrate the effect of PPTr, we first conduct experiments on the 3D Action Recognition task. Followed by P4Transformer, we use the MAR-Action3D dataset which consists of 567 human body point cloud videos, including 20 action categories. Our test/train split follows previous work. Each frame is sampled with 2,048 points. As inputs, point cloud videos are split into multiple clips. Video-level labels are used as clip-level labels during training. In order to estimate the video-level probability, we take the mean of all clip-level probability predictions. We fit the human body point cloud into 4 primitives. 
%In the program calculation, we sort all the points according to the primitive, and divide them into 8 sub-point sets with the same number of points. 
Due to the small scale of human point cloud videos, we can load the entire point cloud videos at one time, so we can avoid maintaining the long-term memory pool in this case. We use the video classification accuracy as the evaluation metric. We compare our method with the latest 4D backbone for point cloud video including MeteorNet, PSTNet and P4Transformer.

% \resizebox{10mm}{5mm}{
% \newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}} 
\begin{table}
\setlength{\tabcolsep}{1mm}
\scriptsize{
\begin{center}
\caption{Evaluation for action recognition on MSR-Action3D dataset~\cite{msr}}
\label{table:msraction3d}
\begin{tabular}{l|c|c|c}
\hline\noalign{\smallskip}
Method & Input & Frames & Accuracy \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
PointNet++~\cite{pointnet2}& point& 1 & 61.61 \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
& point& 4 & 78.11\\
& point& 8 & 81.14\\
MeteorNet~\cite{meteornet}& point& 12 & 86.53\\
& point& 16 & 88.21\\
& point& 24 & 88.50\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
& point& 4 & 81.14\\
& point& 8 & 83.50\\
PSTNet~\cite{pstnet}& point& 12 & 87.88\\
& point& 16 & 89.90\\
& point& 24 & 91.20\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
& point& 4 & 80.11\\
& point& 8 & 83.17\\
P4Transformer~\cite{p4transformer}& point& 12 & 87.54\\
& point& 16 & 89.56\\
& point& 24 & 90.94\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}

& point& 4 & 80.97 \\
& point& 8 & 84.02\\
PPTr(ours)& point&12  & 89.89\\
& point&  16& 90.31\\
& point&  24& \textbf{92.33}\\
\noalign{\smallskip}
\hline

\end{tabular}
\end{center}
}
\end{table}


\textbf{Result.} As reported in Table~\ref{table:msraction3d}, when the number of point cloud frames increases, the classification accuracy can be gradually improved. Our method outperforms all the state-of-the-art methods, demonstrating that our methods can better integrate spacial-temporal information. 


\subsection{Ablation Study and Discussion}
In this section, we first provide an ablation study to verify each component. Then, we provide more analysis to provide an in-depth understanding of our framework.

\subsubsection{Efficacy of intra/inter-primitive Transformer.}
% Ours v.s wo intra-primitive(ongoing) v.s wo inter-primitive(ongoing) v.s. ours-supervoxel v.s. ours-even-partition(ongoing)
We run ablation studies with and without intra/inter-primitive Transformer to quantify its efficacy. We find that PPTr without intra/inter-primitive Transformer results in a $16.73$/$1.39$ accuracy drop on the MSR-Action3D action recognition task. This shows that the intra-primitive transformer is essential in this task. It not only simplifies the optimization difficulty but also aligns similar points, providing good features for the subsequent use of the inter-primitive transformer. Inter-primitive Transformer integrates spatio-temporal information from the entire video, using the complementary information of each frame to further improve classification accuracy.


\subsubsection{Robustness to primitive-fitting hyper-parameters.}

The performance impacts of different numbers of primitives are provided since primitives are crucial in the framework. On MSR-Action3D, we can achieve $91.5$/$91.89$ accuracy with 2/8 primitives, resulting in a marginal drop. On Synthia 4D, the segmentation mIoUs are $82.98$, $84.41$, $84.49$, $84.28$, and $83.56$ with a primitive number of 10, 100, 200, 400, and 2000 respectively. Notice when the primitive number varies in a reasonable range from 100 to 400, the segmentation mIoUs vary by no more than 0.21. When the primitive number is 10, the region division is too coarse for fine-grained segmentation.When the primitive number is 2000, the benefit of the spatial hierarchy gets weakened a lot. The network degenerates to a point transformer when further increasing the primitive number to the point number. This shows that different numbers of primitives have a small effect on the results, and all have consistent improvements.

% \subsubsection{Visualization of attention across videos.}
% In order to explore the associations learned by the primitive transformer, we visualize the points corresponding to the primitives with the largest activation. It can be seen that the primitives corresponding to the limbs and the head have larger activation, indicating that these parts contribute more to the action recognition prediction, which is consistent with common sense and intuition. It is worth mentioning that MSR-Action3D is a single-view point cloud, and the primitives are related to human body shape and actions.
% \begin{figure}[htbp]
%     \centering
%     \vspace{-10pt}
%     \includegraphics[width=8cm]{./figure/attention.png}
%     \vspace{-10pt}
%     \caption{Visualization of attention across videos.}
%     \label{fig:curve}
%     \vspace{-20pt}
% \end{figure}
\subsubsection{Efficacy of primitive representation.}

% We introduce primitive as our middle representation to construct a geometry hierarchy (scene-primitive-point). We compare this design with constructing the hierarchy by even partition. when using even partition as the middle representation, we can achieve the accuracy of $90.8$, which drops $1.53$ on MSR-Action. This result demonstrates that using primitive planes to model the long-term context facilitates optimization and long-term feature association.

Our hierarchical transformer is generic and can be easily applied to mid-level representations other than primitive planes.
To confirm the efficacy of primitive planes, we additionally compare primitive planes with two types of mid-level representations, BPSS~\cite{lin2018toward} supervoxels and k-means clusters.
Results in the table below show that using BPSS supervoxels outperforms P4Transformer but is not as good as using primitive planes while k-means clusters fail to serve as a beneficial mid-level representation on Synthia4D.
\begin{table}[h]
% \vspace{-0.1in}
\begin{center}
\caption{Comparisons between different representations}
\label{table:supervoxel}
\begin{tabular}{ccc}
\hline\noalign{}
 Method & Synthia 4D~\cite{synthia} & MSRAction~\cite{msr} \\
\hline\noalign{}
P4Transformer & 83.16 & 90.94\\\noalign{}
K-means &80.70& 91.76\\\noalign{}
BPSS~\cite{lin2018toward} &83.43&91.98\\\noalign{}
Ours &\textbf{84.49} & \textbf{92.33}\\\noalign{}

\hline
\end{tabular}
\end{center}

\end{table}
\subsubsection{Offline branch and Online branch.} The online branch produces fine primitive features with heavy computation while the offline branch produces coarser features efficiently as a surrogate of the online branch so that the network can process long clips with limited computing resources.
For the action recognition task where data clips can already be largely fit into the GPU memory, using an online branch only with fine primitive features is preferred. In this case, just using an offline branch or combining the offline and online branches results in marginal performance degradation with accuracy of 92.13 and 92.27 respectively. For the 4D segmentation task, using our online branch independently, the memory could only afford 3 frames and the resulting segmentation mIoU(\%) is 84.05. This number goes to 84.49 when assisted by the offline branch covering 30 frames, confirming the value of the offline branch. 
% \subsubsection{Using primitive temporal context v.s. point temporal context (say using 3 frames)}
% \subsubsection{Hyper-parameter of primitive fitting.}



% \begin{figure}[htbp]
%     \centering
%     % \vspace{-10pt}
%     \includegraphics[width=10cm]{./figure/curve.png}
%     % \vspace{-10pt}
%     \caption{Curve of Training process and Occupied memory.}
%     \label{fig:curve}
%     % \vspace{-20pt}
% \end{figure}






==> [ECCV2022] 4DPrimitiveTransformer/tex/introduction.tex <==
% Point cloud videos are ubiquitous in robots and AR systems that act as a window into our dynamically changing 3D world. Being able to record movements in the physical space, point cloud sequences play a key role in comprehending environmental changes and supporting interactions with the world, which can be hardly described by 2D images or static 3D point cloud. Therefore, it's necessary for an intellectual agent to process such form of data precisely to better model the real world, adapt to environmental changes, and interact with them.
% \eric{Need a teaser showing a toy example of using primitives for temporal context.}
% The importance of understanding point cloud videos. - ubiquitous in robots or AR systems and a window into the dynamically changing 3D world. Key for understanding environmental changes and supporting interactions with the world which can be hardly described by static 2D images or 3D point cloud while being more faithful to the physical world than image sequences.
Point cloud videos are ubiquitous in robots and AR systems that act as a window into our dynamically changing 3D world. Being able to record movements in the physical space, point cloud sequences play a key role in comprehending environmental changes and supporting interactions with the world, which can be hardly described by 2D images or static 3D point clouds. Therefore, an intelligent agent must process such a form of data precisely to better model the real world, adapt to environmental changes, and interact with them.

% The challenge of understanding point cloud videos. Effectiveness and efficiency. How to effectively capturing long-term spatial-temporal structure and how to efficiently process long point cloud videos with limited computation resources. 
% Points unstructured, inconsistent across different frames due to camera motion, scene change, the vary of occlusion and sampling patterns, making it hard to effectively integrate different frames well for the underlying spatial-temporal structure. 4D data high dimensional and complex, a naive processing pipeline could easily cause memory and computation explosion. The two challenges both dramatically grow as video length increases.  
Despite its importance, processing point cloud sequences is a quite challenging task for machines that are largely determined by two aspects: effectiveness and efficiency. Effectiveness refers to the ability to capture long-term spatial-temporal structures. Due to camera motion, scene changes, occlusion changes, and sampling patterns, points between different frames are unstructured and inconsistent, making it difficult to effectively integrate different frames into the underlying spatio-temporal structure. Efficiency refers to how to efficiently process long point cloud videos with limited computing resources. The complexity and dimension of 4D data can easily cause memory and computation explosions. Both challenges grow dramatically as the length of the video increases.


% Existing solutions and their limitations. A typical way treats a point cloud video as a 4D volume, directly applies 4D convolution after voxelizing the inputs -  expensive and hard to scale up for large scenes and long sequences. Pure convolution is not very effective at capturing long-term spatial-temporal context compared with recent transformer-based backbones (P4Transformer...). Recent transformer-based 4D backbones do no fully tackle the above two challenges either. still requires loading the whole video sequence into the memory during the learning process, strongly restricting the supported sequence length in large-scale scenes (e.g., XX frames in XX dataset with XX GPU). Moreover, though a flat transformer is able to capture long-term context theoretically, it becomes hard to be optimized as point number increases and usually brings little gain in long videos.
One typical way to tackle the dynamics of point clouds videos is treating the point cloud video as a 4D volume~\cite{minkowski}, which applies 4D convolution directly after voxelization. It is computationally prohibitive when processing large scenes and long videos. Compared with transformer-based 4D backbones, pure convolution is less effective at capturing long-term spatio-temporal context. However, the existing transformer-based 4D backbone(P4Transformer~\cite{p4transformer}) also fails to solve the above challenges. The entire point cloud video still needs to be loaded into memory during the training process, which severely limits the length of the point cloud video (for example, a 24GB graphics card can only handle a synthia4D~\cite{synthia} point cloud video of 3 frames). Additionally, even though flat transformers may be able to capture long-term context theoretically, they are difficult to optimize as point numbers increase and usually do not provide much gain in dense prediction tasks, such as 4D semantic segmentation.


% Our key observations. Long-term context from distant point cloud frames do not need to be on the point-level, not efficient nor effective due to the huge variation of points. A mid-level abstraction spatially descriptive to the underlying geometry and temporally stable is better suited for context modeling. A proper mid-level abstraction not only eases the needs of processing raw points for better efficiency, but also allows easier association across frames for more effective spatial-temporal structure. After revisiting the geometry processing literature, we choose primitive planes as such a mid-level representation, which describes the underlying planar structures in a scene and tends to be much more stabler than raw points across frames.
Based on the challenges described above, we have several key observations. First, considering the large variety of points, distance point cloud frames should not be extracted at the point level, as this is neither efficient nor effective. Second, a middle-level abstraction representing the underlying geometry spatially and temporally can be better suited for context modeling, which will not only alleviate the need to process raw points for better efficiency but also allow for easier association across frames for a more effective spatial-temporal structure. After revisiting the geometry processing literature, we choose primitive plane as a mid-level representation, which describes the underlying planar structures in a scene and tends to be much more stable across frames.



% Our design. We leverage primitive planes to develop an efficient and effective 4D backbone named Point Primitive Transformer (PPTr). As primitive planes induce a natural scene-primitive-point hierarchy in space, we also design PPTr as a hierarchical transformer operating on two different levels as shown in Figure~\ref{}. On the lower level, PPTr extracts short-term spatial-temporal features through an intra-primitive point transformer for a short video clip around the frame of interest. Primitive planes are used to restrict the spatial support of attention maps in a point-level transformer. Such geometry-aware locality inductive bias is not only beneficial for the optimization of transformer but also very effective for extracting descriptive and temporally stable geometric features. On the upper level, PPTr extracts long-term spatial-temporal features through a primitive transformer. We allow very efficient consideration of a long sequence by fitting primitives and compute the primitive features in a pre-processing stage. Through the primitive transformer, we could better associate primitives from different frames and effectively integrate long-term context to the frame of interest.


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{./figure/teaser.pdf}
    \caption{Architecture of Primitive Point Transformer. On the lower level, PPTr extracts short-term spatial-temporal features through an intra-primitive point transformer for a short video clip around the frame of interest. On the upper level, PPTr extracts long-term spatial-temporal features through a primitive transformer.}
    \label{fig:teaser}
    % \vspace{-20pt}
\end{figure}

In this paper, we leverage primitive planes to develop an efficient and effective 4D backbone named Point Primitive Transformer(PPTr). As primitive planes induce a natural scene-primitive-point hierarchy in space, we also design PPTr as a hierarchical transformer operating on two different levels as shown in Figure~\ref{fig:teaser}. On the lower level, PPTr extracts short-term spatial-temporal features through an intra-primitive point transformer for a short video clip around the frame of interest. Primitive planes are used to restrict the spatial support of attention maps in a point-level transformer. Such geometry-aware locality inductive bias is not only beneficial for the optimization of the transformer but also very effective for extracting descriptive and temporally stable geometric features. On the upper level, PPTr extracts long-term spatial-temporal features through a primitive transformer. We allow very efficient consideration of a long sequence by fitting primitives and computing the primitive features in a pre-processing stage. Through the primitive transformer, we could better associate primitives from different frames and effectively integrate long-term context to the frame of interest. 

% Experiments. \eric{Summarize the most impressive experimental results}
We evaluate our Point Primitive Transformer(PPTr) on several tasks, such as 3D action recognition on MSR-Action~\cite{msr} and 4D semantic segmentation on Synthia4D~\cite{synthia} and HOI4D~\cite{liu2022hoi4d}. we demonstrate significant improvements over previous method($+1.33\%$ mIoU on synthia4D, $+6.28\%$ mIoU on HOI4D and $+1.39\%$ accuracy on MSR-Action). 

% Contribution summary. 1. The idea of leveraging primitive plane to capture long-term spatial-temporal context in 4D point cloud videos and a novel backbone named Point Primitive Transformer. 2. An intra-primitive point transformer effective for extracting descriptive and temporally stable short-term geometric features. 3. A primitive transformer efficient for capturing long-term spatial-temporal features. 4. Sota performance?
The contributions of this paper are fourfold:
\begin{itemize}
\item First, we leverage the primitive plane to capture the long-term spatial-temporal context in 4D point cloud videos and propose a novel backbone named Point Primitive Transformer(PPTr). 
\item Second, we propose an intra-primitive point transformer for extracting spatially descriptive and temporally stable \textbf{short-term} geometric features. 
\item Third, we propose a primitive transformer to capture \textbf{long-term} spatial-temporal features efficiently. 
\item Fourth, extensive experiments on three datasets show that the proposed Point Primitive Transformer is more effective and efficient than previous state-of-the-art 4D backbones.
\end{itemize}



==> [ECCV2022] 4DPrimitiveTransformer/tex/method.tex <==
% what, how, why

To develop an efficient and effective backbone for long-term 4D understanding, we draw inspirations from the geometry processing community that primitive planes as some mid-level geometric representations are both compact and stable across time, see Figure~\ref{fig:stableFitting}.
% \eric{Add a figure showing primitives being quite stable across time (does not need to be a complex scene).}
Using primitive planes to model the long-term context not only eases the need to directly deal with the huge number of raw points in a 4D sequence but also facilitates long-term feature association. Furthermore, since primitive planes group points with coherent geometric features, it builds a natural geometry hierarchy (scene-primitive-point) which could be used as a strong inductive bias for powerful yet hard-to-optimize transformer-style architectures. We follow this thought and develop our Point Primitive Transformer. 

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{./figure/stableFitting.pdf}
    % \setlength{\belowcaptionskip}{5cm} 
    \caption{An illustration of primitive fitting in a HOI4D~\cite{liu2022hoi4d} video. Despite changing view angles and challenging interaction, the primitive fitting remains consistent across time.
    }
    \label{fig:stableFitting}
    % \vspace{-10pt}
\end{figure}
Point Primitive Transformer(PPTr) is a two-level hierarchical transformer built upon the geometry hierarchy induced by primitive planes as shown in Figure~\ref{fig:pipeline}. On the lower level, short-term spatial-temporal features are extracted through an intra-primitive point transformer. The intra-primitive point transformer restricts the communication of points within each primitive plane. This design shares a similar flavor with GLOM~\cite{glom} encouraging aligned features to talk. Also due to the local spatial support, it is more friendly to optimization compared with a global transformer. On the upper level, long-term spatial-temporal features are extracted through a primitive transformer. This is done by jointly analyzing short-term features from the lower level and a memory pool storing pre-computed primitive features from a long video. Pre-computed primitive features allow aggregating long-term spatial-temporal context efficiently and effectively. PPTr is very flexible for both point-wise and sequence-wise inference by simply changing the task head.
\begin{figure}[H]
    \centering
     % \vspace{-30pt}
    \includegraphics[width=9cm]{./figure/pipeline.pdf}
    % \vspace{-10pt}
    \caption{Pipeline. The backbone consists of two branches: online network and offline pre-computation. \textbf{1.Online Branch. }The input to network is a short video clip. After primitive fitting, points are tagged with primitive label, then 4D Backbone is applied and generates per-point features. In the  intra-primitive point transformer, points features are enhanced by adapatively adding information from other points inside primitive. Then generate primitive-level representations by maxpooling. In the primitive transformer, clip primitive embeddings(green) perform self-attention with long-term embeddings(yellow) in the memory pool. For semantic segmentation, primitive features are concatenated to corresponding point features then classified into semantic labels. For action recognition, primitive features are merged by maxpooling to a global feature then classified into actions. \textbf{2.Offline Branch. } This branch essentially computes primitive level representations of the long-range videos and maintains a memory pool in an offline manner. After primitive fitting, points are fed to a pre-trained 3D backbone. Then maxpool is applied to every primitive region generating primitive-level embeddings in the memory pool.}
    % \vspace{-20pt}
    \label{fig:pipeline}
\end{figure}
In the rest of this section, we will elaborate on the design of PPTr in detail. We start with how we fit primitive planes and how we pre-compute primitive features in Section~\ref{sec:primitivefitting}. Then in Section~\ref{sec:intra-primitive} and Section~\ref{sec:inter-primitive}, we explain how we extract short-term and long-term spatial-temporal features respectively. 

% Finally we provide additional implementation details in Section~\ref{}.

% In this section, we introduce our design of 4D Hierarchical Primitive Transformer in detail. The input to our network is a point cloud clip $\Psi=\{(P_t, V_t ,F_t)|t=1,\dots,  L\}$, where $P_t$ is the point set of frame $t$ optionally with normal vectors $V_t$, and $F_t$ denotes point features. As illustrated in fig~\ref{fig:pipeline}, we firstly detect primitives for each frame of $\Psi$ and will be described in section~\ref{sec:primitivefitting}. Then we exploit 4D Convolution[] as backbone to obtain per-point features. Next, intra-primitive and inter-primitive transformers are applied to learn relations across space and time in a hierarchical manner, which will be depicted in section~\ref{sec:inter-primitive} and section~\ref{sec:intra-primitive}. Section~\ref{sec:Implementation} provides the details of implementation.
% After a briefly introduction of primitive fitting, we introduce our backbone, 4DHPTransformer, in terms of 4D convolution, intra-primitive attention and inter-primitive attention.   
% \subsection{Overview Architecture}
\label{sec:hierarchicaltransformer}
\subsection{Primitive Fitting and Feature Pre-Computation}
\label{sec:primitivefitting}
% Here we revisit a important problem, Primitive Fitting. Given a point cloud, we need to find out all specific geometries in the point cloud.
We represent a point cloud sequence as $\Psi=\{(P_t, V_t)|t=1,\dots,  L\}$, where $P_t$ is the point cloud of frame $t$ optionally accompanied with normals $V_t$.
In this phase, we detect planes for each frame $(P_t, V_t)$ and output
% For frame $t$, The input is $N$ point coordinates $P_t\in \mathbb{R}^{N\times3}$, optionally normal vectors $V_t\in \mathbb{R}^{N\times3}$,  and the output is the 
primitive label $\Xi_t\in \mathbb{R}^{N\times3}$ and primitive parameters $\Theta_t\in \mathbb{R}^{M\times4}$, where $N$ is the number of points and $M$ is the number of primitives.
We adopt two primitive fitting methods in our study for different datasets: region grow~\cite{regiongrow1} and RANSAC~\cite{ransac}.

We leverage region grow for indoor and outdoor scene segmentation. Region grow detects planes based on normal estimation. If not provided with normal $V_t$, we calculate the normal direction at each point beforehand by linear least squares fitting of a plane over its nearest k neighbors.
% The algorithm can be described as 4 steps. Firstly selects one point from point clouds as a seed item. Secondly employs k nearest neighbor[] to find its neighbors in the data set. Thirdly includes those neighbors which meet the shape requirements. Lastly repeats procedure for every included neighbor until no further neighbor fulfills the requirements. We ensure that newly formed primitive will not conflict with any existing primitive. We use singular value decomposition to determine plane parameter $S=(A, B, C, D)$ where $Ax+By+Cz+D=0$.
Compared with region grow, RANSAC does not require normal estimation and is more suitable for low-resolution point clouds such as those for action recognition in MSR-Action3D~\cite{msr}.
% is more consistent in some sparse scenario like low-resolution point cloud segmentation. We fit 8 planes to each frame of MSR-Action3D[], and the visual effect is illustrated in Fig~\ref{fig:fitting}(b).

After primitive fitting, we pre-compute the primitive features for efficient long-term context aggregation and form a memory pool $F_\text{mem}$ as shown in Figure~\ref{fig:pipeline}. Specifically, we pre-train a 3D point feature learner~\cite{p4transformer} to solve the task of interest just from every  single frame $(P_t,V_t)$. This allows us to extract per-point features $F_t\in\mathbb{R}^{C\times N}$ where $C$ denotes the feature dimension. To extract primitive level representations, point-wise max pooling is adopted for each primitive plane. The final memory pool $F_{\text{mem}}$ has a shape of $\mathbb{R}^{C\times M\times L}$. 



% To better detect primitives on both human body and scenes, we adopt two methods: RANSAC and region grow. 
% \subsubsection{Region grow}
% \label{sec:region grow}detects planes based on normal estimation and excels in scene plane segmentation. If not provided with normal $V_t$, we calculate the normal direction at each point beforehand by linear least squares fitting of a plane over its nearest k neighbors. The algorithm can be described as 4 steps. Firstly selects one point from point clouds as a seed item. Secondly employs k nearest neighbor[] to find its neighbors in the data set. Thirdly includes those neighbors which meet the shape requirements. Lastly repeats procedure for every included neighbor until no further neighbor fulfills the requirements. We ensure that newly formed primitive will not conflict with any existing primitive.\\
% There are 3 requirements for neighbors to be included: accept angle $\alpha$, accept distance $d$ and minimal plane size $n$. Accept angle is the maximum acceptable included angle between plane normal and candidate point normal. Accept distance is the maximum acceptable distance from the point to the estimated plane. Minimal plane size is the minimal number of points to form a plane. If the region ceases growing before reaching minimal size, the whole plane will be discarded and points remain state of undetected. We use Singular Value Decomposition[The singular value decomposition: Its computation and some applications.] to determine plane parameter $S=(A, B, C, D)$ where $Ax+By+Cz+D=0$.\\
% \subsubsection{RANSAC} 
% \label{sec:ransac}
% stands for RANdom SAmple Consensus, a method that iteratively estimates parameters to find the plane with the largest support in the point cloud. Compared with region grow algorithm, RANSAC doesn't require normal estimation, which is more consistent in some sparse scenario like low-resolution point cloud segmentation. We fit 8 planes to each frame of MSR-Action3D[], and the visual effect is illustrated in Fig~\ref{fig:fitting}(b).
% \textbf{TODO: primitive fitting figure of sythia4D HOI4D MSR-Action}\\ 
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=12.3cm]{./figure/primitiveFitting_vis.pdf}
%     \caption{An illustration of Primitive Fitting.  \textbf{a) Region grow on Synthia4D[] and HOI4D[]. } Points with consistent normal direction cluster together. Each primitive region has clear geometric meaning. \textbf{b) RANSAC on MSR-Action3D[]. } Each frame is fitted with 8 planes. Color indicates primitive.}
%     \label{fig:fitting}
% \end{figure}

\subsection{Short-Term Spatial-Temporal Feature Extraction}
% \eric{Add an overall introduction for this branch.}
This branch mainly consists of a 4D backbone and an intra-primitive point transformer.
The per-point features of each 4D sequence are first extracted using the 4D backbone. Following that, an intra-primitive point transformer is used to extract low-level features. Point features can provide the most fine-grained information, enabling us to better perform dense prediction tasks. The intra-primitive point transformer can not only align point features of similar geometry but also save computational overhead and reduce the optimization difficulty of the transformer.

\noindent\textbf{4D Backbone.}
Our 4D backbone is built using a UNet structure. Following the state-of-the-art P4Transformer~\cite{p4transformer}, the encoder/decoder is made up of four 4D convolution/decovolution layers. Given clip $\Psi$, the convolution layer can be described as:\\
\begin{equation}
\begin{aligned}
\boldsymbol{f}_{t}^{\prime(x, y, z)}
% =\sum_{\left(\delta_{x}, \delta_{y}, \delta_{z}, \delta_{t}\right) \in G} \zeta\left(\delta_{x}, \delta_{y}, \delta_{z}, \delta_{t}\right) \cdot \boldsymbol{F}_{t+\delta_{t}}^{\left(x+\delta_{x}, y+\delta_{y}, z+\delta_{z}\right)} \\
% &=\sum_{\delta_{t}=-r_{t}}^{r_{t}} \sum_{\left\|\left(\delta_{x}, \delta_{y}, \delta_{z}\right)\right\| \leq r_{s}} \zeta\left(\delta_{x}, \delta_{y}, \delta_{z}, \delta_{t}\right) \cdot \boldsymbol{F}_{t+\delta_{t}}^{\left(x+\delta_{x}, y+\delta_{y}, z+\delta_{z}\right)} \\
&=\sum_{\delta_{t}=-r_{t}}^{r_{t}} \sum_{\left\|\left(\delta_{x}, \delta_{y}, \delta_{z}\right)\right\| \leq r_{s}} 
(\boldsymbol{W_d}\cdot\left(\delta_{x}, \delta_{y}, \delta_{z}, \delta_{t}\right)^T) \odot(\boldsymbol{W_f} \cdot \boldsymbol{f}_{t+\delta_{t}}^{\left(x+\delta_{x}, y+\delta_{y}, z+\delta_{z}\right)})
\end{aligned}
\end{equation}
where $(x, y, z)\in P_t$ and $(\delta_x, \delta_y,\delta_z,\delta_t)$ is spatial-temporal offset of kernel and $\cdot$ is matrix multiplication. $f_t^{(x, y, z)} \in \mathbb{R}^{C\times1}$ is the feature of point at $(x, y, z, t)$, and the temporal aggregation $\sum$ is implemented with sum-pooling and the spatial $\sum$ is max-pooling. $r_s$ and $r_t$ represent temporal and spatial radius. $\boldsymbol{W_d}\cdot\left(\delta_{x}, \delta_{y}, \delta_{z}, \delta_{t}\right)^T$ generates offset weights where $\boldsymbol{W_d} \in \mathbb{R}^{C'\times 4}$ transforms 4D displacements from $\mathbb{R}^{4\times 1}$ to $\mathbb{R}^{C'\times 1}$, and $\boldsymbol{W_f} \in \mathbb{R}^{C'\times C}$ is a projection matrix. $\odot$ is summation. 

\noindent\textbf{Intra-Primitive Point Transformer.}
\label{sec:intra-primitive}
In this stage, the lower-level feature is extracted by enhancing per-point features obtained from the 4D backbone in a geometry-aware way. point features are clustered in groups according to their primitive labels given in the primitive fitting phase. Compared with simply grouping by k-NN search in euclidean space~\cite{pct}, primitive-based partition has a more underlying geometric meaning such as normal consistency. As point clouds are sets embedded in a metric space, self-attention is a natural way to build connections among them. By optimizing point embeddings in a geometry-aware manner, our intra-primitive transformer takes advantage of local aggregation rather than global information exchange. It is more friendly to optimization than a global transformer because points within the primitive plane cannot communicate with points outside. After this step, points with similar geometric features are easier to align together, which facilitates subsequent higher-level feature extraction. 
\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{./figure/intra.pdf}
    \caption{\textbf{Left: primitive-based region partition.} Points are divided into primitive regions according to primitive labels. Intra-primitive performs self-attention in one primitive region. \textbf{Right: Intra-primitive transformer block.} Consisting of intra-primitive attention layer, pre-LayerNorm~\cite{layernorm}, GELU~\cite{gelu} and residual connection~\cite{resnet}.}
    \label{fig:intra}
    % \vspace{-20pt}
\end{figure}



% if we have more exp results...
Specifically, in the layer $i$, the enhanced point feature $F_{\text{out}}^i$ of primitive region $i$ with input embedding set  $F_{\text{in}}^{i}$ is computed formally as~\cite{attention}:
\begin{equation}
\begin{array}{cc}
     Q= W_q\cdot F_{in}^{i},  K = W_k\cdot F_{in}^{i},  V=W_v\cdot F_{in}^{i} \\
       F_{\text{out}}^{i}=SA( Q,  K,  V) = softmax\left(\frac{ Q^T K}{\sqrt{C^k}}\right)V  \\
    %   F_{out}^{k}=  MLP(LN(SA(LN(F_{in}^{k-1}))+F_{in}^{k-1}))
\end{array}
\end{equation}
where $F_{\text{in}}^i \in \mathbb{R}^{C^i \times N' \times L M}$, $C^i,N',L,M$ represents input dimension, point number per primitive, clip length and primitive number  respectively. $W_q, W_k \in \mathbb{R}^{C^k\times C^i}$, $W_v \in \mathbb{R}^{C^v\times C^i}$ where $C^k$ is the key dimension and $C^v$ is value dimension. $Q, K, V$ are queries, keys and values generated from $F_{in}^{i}$. Attention weights  $softmax\left(\frac{ Q^T K}{\sqrt{C^k}}\right)$ is calculated in the primitive region. The output $F_{\text{out}}^i \in \mathbb{R}^{C^v \times N' \times L M} $ is computed as a weighted sum of the values V. 
% Note that in this section, we only relate $N'$ embeddings that belong to the same primitive of the \textbf{same frame}. We implement this by efficiently reshaping input feature from $\mathbb{R}^{1\times L N' C^i}$ to $\mathbb{R}^{L\times  N' C^i}$[] and assume the first dimension as 'batch dimension'.\\
As shown in Figure~\ref{fig:intra}, we build intra-primitive transformer block with layernorm~\cite{layernorm}, GELU activation~\cite{gelu}, one attentive layer and a following feedforward layer~\cite{attention}. Feedforward is implemented with a two-layer MLP(MultiLayer Perception). % TODO: more detail
% \subsubsection{Memory Pool}
% \label{sec:memorypool}
% stores mid-term representations of primitive region throughout the video, providing complementary long-term information to aid understanding of the current clip. Representations contained in the pool is at primitive level, making long-term point cloud video understanding feasible. After primitive fitting for each frame, we run a 3D backbone[] to acquire point-wise embeddings, then partitioning each frame into regions based on primitives, as demonstrated in Fig\ref{fig:intra}(Left). To extract primitive level representation, point-wise max pool is deployed in every region of video frames. 
% Formally, $M=\{f_{ij}|i=1,\dots,L;j=1,\dots, K\}$ is memory pool which holds a video of $L$ frames, and each frame includes $K$ primitive regions with region features $f$. 
% memory efficient

\subsection{Long-Term Spatial-Temporal Feature Extraction}
\label{sec:inter-primitive}
After the short-term spatial-temporal feature extraction, primitive transformers are used to jointly analyze short-term features from the lower level and a memory pool containing pre-computed primitive features. This branch can not only reduce the computational cost, but also achieve long-term spatio-temporal information integration. 

\noindent\textbf{Primitive Transformer.}
As demonstrated in Fig~\ref{fig:pipeline}, two branches merge here. The output of $l$ layer intra-primitive transformer $F_{out}^l \in \mathbb{R}^{C^l\times N'\times L M}$ is then aggregated by max-pooling operator $MAX\{\cdot \}$ to obtain primitive level feature $F_{out} \in \mathbb{R}^{C^l\times L M}$, where $C^l$ is feature channels, $L$ is the clip length and $M$ is the primitive number. Pre-computed primitive features from memory pool $F_{\text{mem}}$  are used to expand the spatio-temporal receptive field of the primitive transformer. 
Formally, the input of primitive transformer is $F_{\text{in}}^{\text{primitive}} = [F_{\text{clip}} ||  F_{\text{mem}}] \in \mathbb{R}^{C^l\times (L'+L)M}$ which concatenates short-term primitive features $F_{\text{clip}}$ and  primitive features from memory pool $F_{\text{mem}}$. Note that in the primitive attention layer, spatial-temporal attentive aggregation is performed in $(L'+L)\times M$ primitive regions simultaneously. Identical to intra-primitive shown in Fig~\ref{fig:intra}(Right), primitive transformer block is also composed of pre-LayerNorm, primitive attention layer, GELU, feedforward layer and residual connection. 
For semantic segmentation, we concatenate per-point features, intra-primitive point features, and primitive features to obtain point-wise features, and fuse them by a three-layer MLP. For the action recognition task, we use the primitive feature to obtain classification predictions through max-pooling and MLP.
% \subsubsection{Semantic segmentation}
% % 1. depict segmentation and recognition
% % 2. 4D backbone and 3D backbone
% \label{sec:segmentation}
% For semantic segmentation, the input is clip $\Psi=\{(P_t, V_t ,F_t)|t=1,\dots,c,\dots, L\}$ and the output is the predicted semantic label $l_c$ of frame $c$. We concatenate embeddings of frame $c$ fused by intra-primitive transformer with point-wise feature of frame $c$. Formally, suppose $f_i$ is features of point $i$ extracted by backbone and $e_j$ is the embedding of primitive region $j$. Define $primitive(i) \in [1, M]$ that maps point $i$ to primitive region $j$, and $M$ is the number of region in frame $c$. The output semantic label of point $i$ can be described as $$l_c^i = \zeta([f_i || e_j])$$ where $j = primitive(i)$. And we implement function $\zeta(\cdot)$ with three MLP layers.

% \subsubsection{Action Recognition}
% \label{sec:recognition}

% ViViT: A Video Vision Transformer


==> [ECCV2022] 4DPrimitiveTransformer/tex/method_old.tex <==
% what, how, why

To develop an efficient and effective backbone for long-term 4D understanding, we draw inspirations from the geometry processing community that primitive planes as some mid-level geometric representations are both compact and stable across time, see Figure~\ref{fig:stableFitting}.\eric{Add a figure showing primitives being quite stable across time (does not need to be a complex scene).} Using primitive planes to model the long-term context not only eases the needs of directly dealing with the huge number of raw points in a 4D sequence but also facilitates long-term feature association. Furthermore, since primitive planes group points with coherent geometric features, it builds a natural geometry hierarchy (scene-primitive-point) which could be used as a strong inductive bias for powerful yet hard-to-optimize transformer-style architectures. We follow this thought and develop our Point Primitive Transformer (PPTr). 

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{./figure/stableFitting.pdf}
    \caption{An illustration of primitive fitting in a HOI4D[] video. Despite changing view angles and challenging interaction, the primitive fitting remains consistent across time.
    }
    \label{fig:stableFitting}
    % \vspace{-20pt}
\end{figure}
PPTr is a two-level hierarchical transformer build upon the geometry hierarchy induced by primitive planes as shown in Figure~\ref{fig:pipeline}. On the lower level, short-term spatial-temporal features are extracted through an intra-primitive point transformer. The intra-primitive point transformer restricts the communication of points within each primitive plane. This design shares a similar flavor with GLOM~\cite{} encouraging aligned features to talk. Also due to the local spatial support, it is more friendly to optimization compared with a global transformer. On the upper level, long-term spatial-temporal features are extracted through a primitive transformer. This is done by jointly analyzing short-term features from the lower level and a memory pool storing pre-computed primitive features from a long video. Pre-computed primitive features allows aggregating long-term spatial-temporal context efficiently and effectively. PPTr is very flexible for both point-wise and sequence-wise inference by simply changing the task head.

In the rest of this section, we will elaborate the design of PPTr in detail. We start with how we fit primitive planes and how we pre-compute primitive features in Section~\ref{sec:primitivefitting}. Then in Section~\ref{sec:intra-primitive} and Section~\ref{sec:inter-primitive}, we explain how we extract short-term and long-term spatial-temporal features respectively. Finally we provide additional implementation details in Section~\ref{}.

% In this section, we introduce our design of 4D Hierarchical Primitive Transformer in detail. The input to our network is a point cloud clip $\Psi=\{(P_t, V_t ,F_t)|t=1,\dots,  L\}$, where $P_t$ is the point set of frame $t$ optionally with normal vectors $V_t$, and $F_t$ denotes point features. As illustrated in fig~\ref{fig:pipeline}, we firstly detect primitives for each frame of $\Psi$ and will be described in section~\ref{sec:primitivefitting}. Then we exploit 4D Convolution[] as backbone to obtain per-point features. Next, intra-primitive and inter-primitive transformers are applied to learn relations across space and time in a hierarchical manner, which will be depicted in section~\ref{sec:inter-primitive} and section~\ref{sec:intra-primitive}. Section~\ref{sec:Implementation} provides the details of implementation.
% After a briefly introduction of primitive fitting, we introduce our backbone, 4DHPTransformer, in terms of 4D convolution, intra-primitive attention and inter-primitive attention.   

\iffalse
\begin{figure}[t]
    \centering
    \includegraphics[width=12.3cm]{./figure/dataflow.pdf}
    \caption{Dataflow of our pipeline.  \textbf{1. }Input: a video clip of $L$ frames, each frame comprises $N$ points with $F$ feature channels. After primitive fitting, points are tagged with primitive label. Color indicates primitive \textbf{2. }4D Backbone is applied to point set and generate per-point features of $C$ channels. \textbf{3.}Points of same primitives are grouped into primitive regions. Intra-primitive transformer is then applied to these region in parallel. \textbf{4. }Transform local point features into compact embeddings by maxpooling. \textbf{5. }Inter-primitive attention is performed in embeddings of clip and memory pool together. For simplicity, only part of attention(red line) is drawn. \textbf{6.} For semantic segmentation, primitive features are concatenated to corresponding point features then classified into semantic labels. For action recognition, primitive features are merged by maxpooling to a global feature then classified into actions.}
    \label{fig:dataflow}
\end{figure}
\fi

% \subsection{Overview Architecture}
\label{sec:hierarchicaltransformer}

\begin{figure}[t]
    \centering
    \includegraphics[width=12cm]{./figure/pipeline.pdf}
    \caption{Pipeline.  TODO}
    \label{fig:pipeline}
\end{figure}
\subsection{Primitive Fitting and Feature Pre-Computation}
\label{sec:primitivefitting}
% Here we revisit a important problem, Primitive Fitting. Given a point cloud, we need to find out all specific geometries in the point cloud.
We represent a point cloud sequence as $\Psi=\{(P_t, V_t)|t=1,\dots,  L\}$, where $P_t$ is the point cloud of frame $t$ optionally accompanied with normals $V_t$.
In this phase, we detect planes for each frame $(P_t, V_t)$ and output
% For frame $t$, The input is $N$ point coordinates $P_t\in \mathbb{R}^{N\times3}$, optionally normal vectors $V_t\in \mathbb{R}^{N\times3}$,  and the output is the 
primitive label $\Xi_t\in \mathbb{R}^{N\times3}$ and primitive parameters $\Theta_t\in \mathbb{R}^{M\times4}$, where $N$ is the number of points and $M$ is the number of primitives.
We adopt two primitive fitting methods in our study for different datasets: region grow~\cite{} and RANSAC~\cite{}.

We leverage region grow for indoor and outdoor scene segmentation. Region grow detects planes based on normal estimation. If not provided with normal $V_t$, we calculate the normal direction at each point beforehand by linear least squares fitting of a plane over its nearest k neighbors.
% The algorithm can be described as 4 steps. Firstly selects one point from point clouds as a seed item. Secondly employs k nearest neighbor[] to find its neighbors in the data set. Thirdly includes those neighbors which meet the shape requirements. Lastly repeats procedure for every included neighbor until no further neighbor fulfills the requirements. We ensure that newly formed primitive will not conflict with any existing primitive. We use singular value decomposition to determine plane parameter $S=(A, B, C, D)$ where $Ax+By+Cz+D=0$.
Compared with region grow, RANSAC does not require normal estimation and is more suitable for low-resolution point clouds such as those for action recognition in MSR-Action3D~\cite{}.
% is more consistent in some sparse scenario like low-resolution point cloud segmentation. We fit 8 planes to each frame of MSR-Action3D[], and the visual effect is illustrated in Fig~\ref{fig:fitting}(b).

After primitive fitting, we pre-compute the primitive features for efficient long-term context aggregation and form a memory pool $F_\text{mem}$ as shown in Figure~\ref{fig:pipeline}. Specifically, we pre-train a 3D point feature learner~\cite{} to solve the task of interest just from each single frame $(P_t,V_t)$. This allows us to extract per-point features $F_t\in\mathbb{R}^{N\times C}$ where $C$ denotes the feature dimension. To extract primitive level representations, point-wise max pooling is adopted for each primitive plane. The final memory pool $F_{\text{mem}}$ has a shape of $\mathbb{R}^{M\times L\times C}$. 



% To better detect primitives on both human body and scenes, we adopt two methods: RANSAC and region grow. 
% \subsubsection{Region grow}
% \label{sec:region grow}detects planes based on normal estimation and excels in scene plane segmentation. If not provided with normal $V_t$, we calculate the normal direction at each point beforehand by linear least squares fitting of a plane over its nearest k neighbors. The algorithm can be described as 4 steps. Firstly selects one point from point clouds as a seed item. Secondly employs k nearest neighbor[] to find its neighbors in the data set. Thirdly includes those neighbors which meet the shape requirements. Lastly repeats procedure for every included neighbor until no further neighbor fulfills the requirements. We ensure that newly formed primitive will not conflict with any existing primitive.\\
% There are 3 requirements for neighbors to be included: accept angle $\alpha$, accept distance $d$ and minimal plane size $n$. Accept angle is the maximum acceptable included angle between plane normal and candidate point normal. Accept distance is the maximum acceptable distance from the point to the estimated plane. Minimal plane size is the minimal number of points to form a plane. If the region ceases growing before reaching minimal size, the whole plane will be discarded and points remain state of undetected. We use Singular Value Decomposition[The singular value decomposition: Its computation and some applications.] to determine plane parameter $S=(A, B, C, D)$ where $Ax+By+Cz+D=0$.\\
% \subsubsection{RANSAC} 
% \label{sec:ransac}
% stands for RANdom SAmple Consensus, a method that iteratively estimates parameters to find the plane with the largest support in the point cloud. Compared with region grow algorithm, RANSAC doesn't require normal estimation, which is more consistent in some sparse scenario like low-resolution point cloud segmentation. We fit 8 planes to each frame of MSR-Action3D[], and the visual effect is illustrated in Fig~\ref{fig:fitting}(b).
% \textbf{TODO: primitive fitting figure of sythia4D HOI4D MSR-Action}\\ 
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=12.3cm]{./figure/primitiveFitting_vis.pdf}
%     \caption{An illustration of Primitive Fitting.  \textbf{a) Region grow on Synthia4D[] and HOI4D[]. } Points with consistent normal direction cluster together. Each primitive region has clear geometric meaning. \textbf{b) RANSAC on MSR-Action3D[]. } Each frame is fitted with 8 planes. Color indicates primitive.}
%     \label{fig:fitting}
% \end{figure}

\subsection{Short-Term Feature Extraction}
\eric{Add an overall introduction for this branch.}

\noindent\textbf{4D Backbone}
We implement our 4D backbone with UNet structure to extract point feature of video. Following the state-of-the-art P4Transformer[], the encoder/decoder is made up of four 4D convolution/decovolution layers. Given clip $\Psi$, the convolution layer can be described as:\\
\begin{equation}
\begin{aligned}
\boldsymbol{f}_{t}^{\prime(x, y, z)}
% =\sum_{\left(\delta_{x}, \delta_{y}, \delta_{z}, \delta_{t}\right) \in G} \zeta\left(\delta_{x}, \delta_{y}, \delta_{z}, \delta_{t}\right) \cdot \boldsymbol{F}_{t+\delta_{t}}^{\left(x+\delta_{x}, y+\delta_{y}, z+\delta_{z}\right)} \\
% &=\sum_{\delta_{t}=-r_{t}}^{r_{t}} \sum_{\left\|\left(\delta_{x}, \delta_{y}, \delta_{z}\right)\right\| \leq r_{s}} \zeta\left(\delta_{x}, \delta_{y}, \delta_{z}, \delta_{t}\right) \cdot \boldsymbol{F}_{t+\delta_{t}}^{\left(x+\delta_{x}, y+\delta_{y}, z+\delta_{z}\right)} \\
&=\sum_{\delta_{t}=-r_{t}}^{r_{t}} \sum_{\left\|\left(\delta_{x}, \delta_{y}, \delta_{z}\right)\right\| \leq r_{s}} 
(\boldsymbol{W_d}\cdot\left(\delta_{x}, \delta_{y}, \delta_{z}, \delta_{t}\right)^T) \odot(\boldsymbol{W_f} \cdot \boldsymbol{f}_{t+\delta_{t}}^{\left(x+\delta_{x}, y+\delta_{y}, z+\delta_{z}\right)})
\end{aligned}
\end{equation}
where $(x, y, z)\in P_t$ and $(\delta_x, \delta_y,\delta_z,\delta_t)$ is spatial-temporal offset of kernel and $\cdot$ is matrix multiplication. $f_t^{(x, y, z)} \in \mathbb{R}^{C\times1}$ is the feature of point at $(x, y, z, t)$, and the temporal aggregation $\sum$ is implemented with sum-pooling and the spatial $\sum$ is max-pooling. $r_s$ and $r_t$ represent temporal and spatial radius. $\boldsymbol{W_d}\cdot\left(\delta_{x}, \delta_{y}, \delta_{z}, \delta_{t}\right)^T$ generates offset weights where $\boldsymbol{W_d} \in \mathbb{R}^{C'\times 4}$ transforms 4D displacements from $\mathbb{R}^{4\times 1}$ to $\mathbb{R}^{C'\times 1}$, and $\boldsymbol{W_f} \in \mathbb{R}^{C'\times C}$ is a projection matrix. $\odot$ is summation. 

\noindent\textbf{Intra-Primitive Transformer}
\label{sec:intra-primitive}
is designed to enhance point features obtained from 4D Convolution[] in a geometry-aware way. Because point clouds are essentially sets embedded in a metric space, self-attention fits naturally for building connections between them. Instead of facilitating information exchange globally, our intra-primitive transformer adopts local aggregation strategy[] to optimize the point embeddings in a geometry-aware way. As shown in Figure~\ref{fig:dataflow}, point features are clustered in groups according to their primitive labels given in primitive fitting phase. Compared with simply grouping by k-NN search in euclidean space[], primitive-based partition has more underlying geometric meaning such as normal consistency. And it additionally enlarges receptive fields by reaching farther points that belonging to the primitive. 

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{./figure/intra.pdf}
    \caption{\textbf{Left: primitive-based region partition.} Points are divided into primitive regions according to primitive labels. Intra-primitive performs self-attention in one primitive region. \textbf{Right: Intra-primitive transformer block.} Consisting of intra-primitive attention layer, pre-LayerNorm, GELU and residual connection.}
    \label{fig:intra}
    % \vspace{-20pt}
\end{figure}

% if we have more exp results...
Specifically, in the layer $i$, the fused feature $F_{out}^i$ of primitive region $i$ with input embedding set  $F_{in}^{i}$ is computed formally as[]:
\begin{equation}
\begin{array}{cc}
     Q= W_q\cdot F_{in}^{i},  K = W_k\cdot F_{in}^{i},  V=W_v\cdot F_{in}^{i} \\
       F_{out}^{i}=SA( Q,  K,  V) = softmax\left(\frac{ Q^T K}{\sqrt{C^k}}\right)V  \\
    %   F_{out}^{k}=  MLP(LN(SA(LN(F_{in}^{k-1}))+F_{in}^{k-1}))
\end{array}
\end{equation}
where $F_{in}^i \in \mathbb{R}^{1\times L\cdot N'\cdot C^i}$, $ L,N',C^i$ represents clip length, point number and input dimension respectively. $W_q, W_k \in \mathbb{R}^{C^k\times C^i}$, $W_k \in \mathbb{R}^{C^v\times C^i}$ where $C^k$ is the key dimension and $C^v$ is value dimension. $Q, K, V$ are queries, keys and values generated from $F_{in}^{i}$. Attention weights  $softmax\left(\frac{ Q^T K}{\sqrt{C^k}}\right)$ is calculated in the primitive region. Note that in this section, we only relate $N'$ embeddings that belong to the same primitive of the \textbf{same frame}. We implement this by efficiently reshaping input feature from $\mathbb{R}^{1\times L N' C^i}$ to $\mathbb{R}^{L\times  N' C^i}$[] and assume the first dimension as 'batch dimension'.\\
As shown in Figure~\ref{fig:intra}, we build intra-primitive transformer block with layernorm, GELU activation, one attentive layer and a following feedforward layer. Feedforward is implemented with a two-layer MLP(Multilayer perception). % TODO: more detail
The output of $l$ layer intra-primitive transformer $F_{out}^l \in \mathbb{R}^{LC^l\times N'}$ is then aggregated by vector max operator $MAX\{\cdot \}$ to obtain primitive level feature $F_{out} \in \mathbb{R}^{LC^l\times 1}$.
% \subsubsection{Memory Pool}
% \label{sec:memorypool}
% stores mid-term representations of primitive region throughout the video, providing complementary long-term information to aid understanding of the current clip. Representations contained in the pool is at primitive level, making long-term point cloud video understanding feasible. After primitive fitting for each frame, we run a 3D backbone[] to acquire point-wise embeddings, then partitioning each frame into regions based on primitives, as demonstrated in Fig\ref{fig:intra}(Left). To extract primitive level representation, point-wise max pool is deployed in every region of video frames. 
% Formally, $M=\{f_{ij}|i=1,\dots,L;j=1,\dots, K\}$ is memory pool which holds a video of $L$ frames, and each frame includes $K$ primitive regions with region features $f$. 
% memory efficient

\subsection{Long-Term Feature}
\label{sec:architecture}
% In this section, we illustrate the core design of hierarchical primitive transformer.

\subsubsection{Inter-Primitive Transformer}
\label{sec:inter-primitive}
is proposed to adaptively combine primitive-level representations from different primitive regions across the video. As demonstrated in Fig~\ref{fig:pipeline}, two streams of embeddings merge here. Fused by intra-primitive transformer, short-term embeddings are of size $M\times L$, where $M$ is the number of primitive region in single frame and $L$ is the clip length. Long-term embeddings support understanding of short-term clip by increasing frame size $L'$ of memory pool. In this fashion, inter-primitive transformer is capable of learning long-term context when processing the current clip. Formally, the input of inter-primitive transformer is $F_{in}^{inter} = [F_{clip} ||  F_{mem}] \in \mathbb{R}^{BC^lM\times (L'+L)}$ which concatenates clip features $F_{clip}$ and long-term features $F_{mem}$. Note that in the inter-primitive attention layer, spatial-temporal attentive aggregation is performed in $M\times(L'+L)$ primitive regions simultaneously. Identical to intra-primitive shown in Fig~\ref{fig:intra}(Right), inter-primitive transformer block is composed of pre-LayerNorm, inter-primitive attention layer, GELU, feedforward layer and residual connection. 

\subsubsection{Semantic segmentation}
% 1. depict segmentation and recognition
% 2. 4D backbone and 3D backbone
\label{sec:segmentation}
For semantic segmentation, the input is clip $\Psi=\{(P_t, V_t ,F_t)|t=1,\dots,c,\dots, L\}$ and the output is the predicted semantic label $l_c$ of frame $c$. We concatenate embeddings of frame $c$ fused by intra-primitive transformer with point-wise feature of frame $c$. Formally, suppose $f_i$ is features of point $i$ extracted by backbone and $e_j$ is the embedding of primitive region $j$. Define $primitive(i) \in [1, M]$ that maps point $i$ to primitive region $j$, and $M$ is the number of region in frame $c$. The output semantic label of point $i$ can be described as $$l_c^i = \zeta([f_i || e_j])$$ where $j = primitive(i)$. And we implement function $\zeta(\cdot)$ with three MLP layers.

\subsubsection{Action Recognition}
\label{sec:recognition}

% ViViT: A Video Vision Transformer


==> [ECCV2022] 4DPrimitiveTransformer/tex/pilot.tex <==
4D point cloud video understanding has obtained much attention recently and researchers are actively seeking for backbones to capture descriptive spatial-temporal features. Among them, P4Transformer~\cite{p4transformer} is the leading one achieving state-of-the-art performance on common tasks including 4D semantic segmentation and 4D action recognition. Briefly speaking, instead of tracking points, P4Transformer uses a point 4D convolution to encode the spatio-temporal local structures in a point cloud video, and utilize the transformer to capture the global appearance and motion information across the entire video.
% \eric{Please summarize P4Transformer briefly here.}
% Existing works on point cloud video analysis mainly focus on MSRaction3D, a dataset for action recognition task. The current state-of-the-art work in this area is P4Transformer which introduces a global transformer to capture spatial-temporal information.
To motivate the necessity of a new backbone, we conduct a pilot study to understand the constraints of P4Transformer for long-term point cloud video understanding. 
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{./figure/pilot.png}
    \vspace{-10pt}
     \caption{\textbf{(a)} The performance gain(MSR-Action3D~\cite{msr}) with the increase of temporal range. \textbf{(b)} The occupied memory with the increase of temporal range. We take the 2080Ti(11GB) GPU as an example. When the GPU memory cap is reached, the maximum number of frames that can be used is 15, which can only achieve $89\%$ accuracy. }
    \label{fig:pilot}
    \vspace{-10pt}
\end{figure}
\begin{itemize}
    \item We first experiment with the action recognition task on MSR-Action3D~\cite{msr} dataset. We gradually increase the clip length until our GPU memory cap is reached and examine how well P4transformer performs.
    % and how transformer contributes to the final performance.
    The results are shown in Figure~\ref{fig:pilot}. 
    \item We further conduct 4D semantic segmentation experiments on the synthia 4D dataset~\cite{synthia}, to verify the effect of Transformer. Specifically, We removed the Transformer in P4Transformer and compared it with the full version.
\end{itemize}

We can draw mainly two conclusions from the above experiments. First, as shown in Figure~\ref{fig:pilot}, P4Transformer achieves better performance as the clip length increases but is soon restricted by the huge memory cost, and it is hard to apply P4Transformer to very long clips. When the GPU memory cap is reached, the performance still keeps its trend of going up, indicating the huge potential of exploring longer-term videos. 
Second, in synthia4D~\cite{synthia} semantic segmentation task, we find that P4transformer without Transformer can achieve mIoU of $80.3\%$, which only drops $2.86\%$ compared with original P4Transformer. This result indicates global spatial-temporal context captured by P4Transformer becomes less useful in 4D dense prediction tasks. This is quite counter-intuitive as the first conclusion indicates the benefit of modeling long-term information. We conjecture that using a flat transformer as in P4Transformer is not effective for long-term spatial-temporal context due to optimization issues.

% In Figure~\ref{fig:polit}, we show how global spatial-temporal context captured via transformer contribute to the 
% we show how action recognition accuracy and occupied memory change with the clip length grows. Figure~\ref{fig:polit}(a) shows the classification accuracy increases as the clip length increases. Figure~\ref{fig:polit}(b) shows that the amount of occupied memory increases rapidly, which leads to the clip's length cannot be very long. This problem will be more serious on large-scale point cloud videos. For example, in an outdoor autonomous driving scene, a point cloud video with a clip length of 3 will reach the maximum memory, which makes it impossible to integrate long-term temporal information.\eric{I think we can motivate this with a 2080ti GPU whose memory is 11GB. We should also cut the figure with a memory cap 11G.} \\

We re-examine the design principles of 4D backbones for long-term videos and we would like to emphasize two important properties: efficiency (both speed-wise and memory-wise) and effectiveness. By efficiency, we mean the backbone should be able to effectively model long-term context to understand 4D visual data in a more integrated way. P4Transformer is not efficient since it needs to load a whole point cloud sequence into the memory for per-point feature learning. This could easily explode the memory as the sequence becomes longer or input scenes become larger-scale. Similar drawbacks also apply to most other 4D backbones in the literature. P4Transformer is also not effective enough for aggregating long-term context due to the usage of ball-like region features. P4Transformer samples equal-sized ball regions in each frame to compute feature tokens and applies transformer to a sequence of frames. The geometric meaning of such randomly sampled balls could hugely vary in dynamic scenes. This makes it hard to build long-term associations, which is important for long-term context.

% This makes us rethink the design of 4D neural networks, especially 4D Transformers. We believe that a good 4D point cloud video backbone should have the following two properties: efficient and light-weight.
% P4Transformer demonstrates the potential of transformers, but apparently does not have the above advantages. Among all possible explanations, we highlight two points:\\ 
% \textbf{Video-level attention is inefficient.} Video attention needs to be calculated in the entire point cloud video, which is computationally complex and difficult to optimize. When the clip length is relatively short, the network works well, but when it exceeds a certain threshold, the optimization problem becomes very difficult and there is a risk of memory overflow.\\
% \textbf{No suitable intermediate representation.} When computing attention weights, it is not feasible to use all point features due to computational constraints. P4Transformer~\cite{} uses region features to calculate attention weights, but points within the same region do not necessarily have similar geometric features, and using them as intermediate representations may cause ambiguity.\\
% Therefore, in order to design a better 4D backbone network, we need to find an efficient network architecture that can integrate point cloud videos as long as possible with limited computing resources. We also need to design a suitable intermediate representation to calculate the attention weights, which should have consistent geometric features.\\

==> [ECCV2022] 4DPrimitiveTransformer/tex/relatedwork.tex <==
\noindent{\bf Deep learning on Point Cloud Video Processing.} 
% 1.4D convolution 2.long-term info matters 3.existing methods cannot reach long-term[ViViT]
Different from grid-based RGB video, point cloud video exhibits irregularities and lacks order along the spatial dimension where points emerge inconsistently across time. One approach to deal with that is voxilization. For instance, ~\cite{minkowski} extends temporal dimension to 3D sparse convolution~\cite{spconv} to extract spatial temporal features on 4D occupancy grids. 3DV~\cite{3dv} proposes a 3D motion representation to encode 3D motion information via temporal rank pooling~\cite{rankpool}. Another approach is to perform directly on point sets. MeteorNet~\cite{meteornet} adopts PointNet++~\cite{pointnet2} to aggregate information from neighbors, while point-track is needed to merge points. PSTNet~\cite{pstnet} firstly decomposes spatial and temporal information and proposes a point-based convolution in a hierarchical manner. Following~\cite{pstnet}~\cite{meteornet}, P4Transformer~\cite{p4transformer} proposes 4D Convolution that performs spatial-temporal convolution and captures dynamics of points by self-attention. While like most point-based approaches, they prolong input clip by simply feeding raw points into network, which suffers from limited memory and fails to benefit from long-range temporal dependencies. Based on this, we propose Point Primitive Transformer(PPTr) which enjoys all three properties: point-convolution based, long-term supported and point-track avoided.

% While point cloud video processing is a fairly new task, RGB video processing is a long standing problem. The key is to model inter-frame relationship[]. In RGB video processing, [] extracts single frame feature and learns inter-frame relationship by RNN. 3D CNNs[] are also widely used to learn temporal relation, however they suffer from low temporal dependency. To address that, [,] propose memory pool to learn long-range temporal relations. Our method is \eric{We should just focus on point cloud video processing in this paragraph.}\\
\noindent{\bf Primitive Fitting.} 
% \subsubsection{Primitive Fitting.}
Primitive fitting is a long-standing problem of grouping points into specific geometric shapes such as plane, cuboid, cylinder and so on. Such process approximates and abstracts 3D shapes from low-level digitized point data to a succinct high-level parameterized representation. Two mainstream solutions of primitive fitting in geometry community are RANSAC~\cite{ransac}~\cite{efficientransac} and region grow~\cite{regiongrow1}~\cite{regiongrow2}. Recently, neural networks have been developed by several works~\cite{3dprnn}~\cite{spfn}~\cite{hpnet}~\cite{primitivenet}~\cite{volumetricprimitives} to segment primitives. Because primitives extremely simplifies point data while keeps a relatively precise description of 3D geometry, they are widely applied to downstream tasks like instance segmentation~\cite{primitivenet}, reconstruction~\cite{architecturalmodeling}and animation~\cite{animated}. For example, ~\cite{shapetemplates} utilizes primitive shapes that are rich in underlying structures to reconstruct scanned object and transfer the structural information onto new objects. To directly deal with large-scale scenes, ~\cite{SPG} distils organization of point cloud by partitioning heavy points into light shapes, showing the power of such compact yet rich representation. We inject primitives into our network, intending to spatially provide geometric-aware enhancement on local primitive region and temporally leverage long-range information in a memory efficient way.\\
% Primitive fitting is the task of grouping points into specific geometric shapes, which has been studied considerably in the history. Two main non-learning methods are RANSAC[Random sample consensus: a paradigm for model ﬁtting with applications to image analysis and automated cartography, Efﬁcient ransac for point-cloud shape detection, Globﬁt: Consistently ﬁtting primitives by discovering global relations, Primitive ﬁtting based on the efﬁcient multibaysac algorithm] and region grow[Robust segmentation of primitives from range data in the presence of geometric degeneracy,  Segmentation of point clouds using smoothness constraint]. RANSAC and its variants[] are effective in detecting primitives, which fit models in a iterative way. Schnabel et al. [28] introduced a robust RANSAC-based framework for fitting multiple primitives of different types in point cloud. While these methods perform well in some situation, they're sensitive to hyperparameter and sometimes can be time-consuming. Region grow starts from a seed region with a hypothetical primitive shape and keeps expanding until detection error is beyond threshold. Recently several works[] have developed supervised deep learning models for primitive segmentation. []can fit  input shape with cuboids, and []support more variety of shapes. For a more comprehensive review with regard to primitive fitting, please refer to []. We choose region grow because compared with RANSAC and learning-based method, it's more robust to parameter adjustments and faster.\eric{Related work here should focus more on the usage of primitives in different deep learning applications. The computation methodology should only be mentioned briefly.}\\
% {\bf Deep learning on 3D point clouds.} 
% % \subsubsection{Deep learning on 3D point clouds.}
% Deep learning is now widely used in 3D point cloud processing such as semantic segmentation~\cite{pointnet}~\cite{pointnet2}~\cite{kpconv}~\cite{pointconv}, detection~\cite{detection1}~\cite{detection2}~\cite{detection3}, reconstruction~\cite{reconstruction1}~\cite{reconstruction2} and so on. PointNet~\cite{pointnet} pioneers point-based method, which directly operates on unordered point clouds and construct a symmetric function with shared-weight deep neural network to generate per-point feature. PointNet++~\cite{pointnet2} is its follow-up work, where local features of point set are extracted and aggregated hierarchically. However, these methods apply only to static 3D point clouds, which is unable to process point cloud videos.\\
% \eric{This paragraph could be either keep or removed dependent on the space constraints.}\\
% \subsubsection{Deep learning on RGB and Point Cloud Video.}
% \subsubsection{Transformer Network.}
{\bf Transformer Network.} 
Transformer is a powerful deep neural network based on self-attention mechanism~\cite{attention} and is particularly suitable for modelling long-range dependencies~\cite{nlp1}~\cite{nlp2}~\cite{nlp3}. It was firstly proposed in~\cite{attention} for machine translation task and further extended to vision community~\cite{vivit}~\cite{nonlocal3}~\cite{vit}~\cite{vit2}~\cite{nonlocal1}~\cite{nonlocal2}~\cite{nonlocal4} . Very recently, Swin Transformer~\cite{swin} proposes a hierarchical design for vision modeling at various scales and yields impressive results . Similar to CNNs~\cite{cnn1}~\cite{resnet}, Swin transformer builds hierarchical feature maps by merging image patches when layers go deeper, and strikes a balance between efficiency and effectiveness by limiting self-attention to local windows while also supporting cross-window connection. In 4D point cloud understanding, prior leading work~\cite{p4transformer} performs self-attention globally and fails to leverage long-term dependencies effectively. As such, we design a hierarchical Primitive Point Transformer(PPTr) to alleviate ineffectiveness of global-wise attention and introduce intra-primitive point transformer and primitive transformer that perform self-attention at point level and primitive level respectively. Intensive experiments have shown that our network outperforms the state-of-the-art methods for both 4D semantic segmentation and 4D action recognition.
% \eric{We should talk about Swin Transformer and other hierarchical designs and highlight the importance of how to build the hierarchy.}

==> tex/method_old.tex <==
% what, how, why

To develop an efficient and effective backbone for long-term 4D understanding, we draw inspirations from the geometry processing community that primitive planes as some mid-level geometric representations are both compact and stable across time, see Figure~\ref{fig:stableFitting}.\eric{Add a figure showing primitives being quite stable across time (does not need to be a complex scene).} Using primitive planes to model the long-term context not only eases the needs of directly dealing with the huge number of raw points in a 4D sequence but also facilitates long-term feature association. Furthermore, since primitive planes group points with coherent geometric features, it builds a natural geometry hierarchy (scene-primitive-point) which could be used as a strong inductive bias for powerful yet hard-to-optimize transformer-style architectures. We follow this thought and develop our Point Primitive Transformer (PPTr). 

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{./figure/stableFitting.pdf}
    \caption{An illustration of primitive fitting in a HOI4D[] video. Despite changing view angles and challenging interaction, the primitive fitting remains consistent across time.
    }
    \label{fig:stableFitting}
    % \vspace{-20pt}
\end{figure}
PPTr is a two-level hierarchical transformer build upon the geometry hierarchy induced by primitive planes as shown in Figure~\ref{fig:pipeline}. On the lower level, short-term spatial-temporal features are extracted through an intra-primitive point transformer. The intra-primitive point transformer restricts the communication of points within each primitive plane. This design shares a similar flavor with GLOM~\cite{} encouraging aligned features to talk. Also due to the local spatial support, it is more friendly to optimization compared with a global transformer. On the upper level, long-term spatial-temporal features are extracted through a primitive transformer. This is done by jointly analyzing short-term features from the lower level and a memory pool storing pre-computed primitive features from a long video. Pre-computed primitive features allows aggregating long-term spatial-temporal context efficiently and effectively. PPTr is very flexible for both point-wise and sequence-wise inference by simply changing the task head.

In the rest of this section, we will elaborate the design of PPTr in detail. We start with how we fit primitive planes and how we pre-compute primitive features in Section~\ref{sec:primitivefitting}. Then in Section~\ref{sec:intra-primitive} and Section~\ref{sec:inter-primitive}, we explain how we extract short-term and long-term spatial-temporal features respectively. Finally we provide additional implementation details in Section~\ref{}.

% In this section, we introduce our design of 4D Hierarchical Primitive Transformer in detail. The input to our network is a point cloud clip $\Psi=\{(P_t, V_t ,F_t)|t=1,\dots,  L\}$, where $P_t$ is the point set of frame $t$ optionally with normal vectors $V_t$, and $F_t$ denotes point features. As illustrated in fig~\ref{fig:pipeline}, we firstly detect primitives for each frame of $\Psi$ and will be described in section~\ref{sec:primitivefitting}. Then we exploit 4D Convolution[] as backbone to obtain per-point features. Next, intra-primitive and inter-primitive transformers are applied to learn relations across space and time in a hierarchical manner, which will be depicted in section~\ref{sec:inter-primitive} and section~\ref{sec:intra-primitive}. Section~\ref{sec:Implementation} provides the details of implementation.
% After a briefly introduction of primitive fitting, we introduce our backbone, 4DHPTransformer, in terms of 4D convolution, intra-primitive attention and inter-primitive attention.   

\iffalse
\begin{figure}[t]
    \centering
    \includegraphics[width=12.3cm]{./figure/dataflow.pdf}
    \caption{Dataflow of our pipeline.  \textbf{1. }Input: a video clip of $L$ frames, each frame comprises $N$ points with $F$ feature channels. After primitive fitting, points are tagged with primitive label. Color indicates primitive \textbf{2. }4D Backbone is applied to point set and generate per-point features of $C$ channels. \textbf{3.}Points of same primitives are grouped into primitive regions. Intra-primitive transformer is then applied to these region in parallel. \textbf{4. }Transform local point features into compact embeddings by maxpooling. \textbf{5. }Inter-primitive attention is performed in embeddings of clip and memory pool together. For simplicity, only part of attention(red line) is drawn. \textbf{6.} For semantic segmentation, primitive features are concatenated to corresponding point features then classified into semantic labels. For action recognition, primitive features are merged by maxpooling to a global feature then classified into actions.}
    \label{fig:dataflow}
\end{figure}
\fi

% \subsection{Overview Architecture}
\label{sec:hierarchicaltransformer}

\begin{figure}[t]
    \centering
    \includegraphics[width=12cm]{./figure/pipeline.pdf}
    \caption{Pipeline.  TODO}
    \label{fig:pipeline}
\end{figure}
\subsection{Primitive Fitting and Feature Pre-Computation}
\label{sec:primitivefitting}
% Here we revisit a important problem, Primitive Fitting. Given a point cloud, we need to find out all specific geometries in the point cloud.
We represent a point cloud sequence as $\Psi=\{(P_t, V_t)|t=1,\dots,  L\}$, where $P_t$ is the point cloud of frame $t$ optionally accompanied with normals $V_t$.
In this phase, we detect planes for each frame $(P_t, V_t)$ and output
% For frame $t$, The input is $N$ point coordinates $P_t\in \mathbb{R}^{N\times3}$, optionally normal vectors $V_t\in \mathbb{R}^{N\times3}$,  and the output is the 
primitive label $\Xi_t\in \mathbb{R}^{N\times3}$ and primitive parameters $\Theta_t\in \mathbb{R}^{M\times4}$, where $N$ is the number of points and $M$ is the number of primitives.
We adopt two primitive fitting methods in our study for different datasets: region grow~\cite{} and RANSAC~\cite{}.

We leverage region grow for indoor and outdoor scene segmentation. Region grow detects planes based on normal estimation. If not provided with normal $V_t$, we calculate the normal direction at each point beforehand by linear least squares fitting of a plane over its nearest k neighbors.
% The algorithm can be described as 4 steps. Firstly selects one point from point clouds as a seed item. Secondly employs k nearest neighbor[] to find its neighbors in the data set. Thirdly includes those neighbors which meet the shape requirements. Lastly repeats procedure for every included neighbor until no further neighbor fulfills the requirements. We ensure that newly formed primitive will not conflict with any existing primitive. We use singular value decomposition to determine plane parameter $S=(A, B, C, D)$ where $Ax+By+Cz+D=0$.
Compared with region grow, RANSAC does not require normal estimation and is more suitable for low-resolution point clouds such as those for action recognition in MSR-Action3D~\cite{}.
% is more consistent in some sparse scenario like low-resolution point cloud segmentation. We fit 8 planes to each frame of MSR-Action3D[], and the visual effect is illustrated in Fig~\ref{fig:fitting}(b).

After primitive fitting, we pre-compute the primitive features for efficient long-term context aggregation and form a memory pool $F_\text{mem}$ as shown in Figure~\ref{fig:pipeline}. Specifically, we pre-train a 3D point feature learner~\cite{} to solve the task of interest just from each single frame $(P_t,V_t)$. This allows us to extract per-point features $F_t\in\mathbb{R}^{N\times C}$ where $C$ denotes the feature dimension. To extract primitive level representations, point-wise max pooling is adopted for each primitive plane. The final memory pool $F_{\text{mem}}$ has a shape of $\mathbb{R}^{M\times L\times C}$. 



% To better detect primitives on both human body and scenes, we adopt two methods: RANSAC and region grow. 
% \subsubsection{Region grow}
% \label{sec:region grow}detects planes based on normal estimation and excels in scene plane segmentation. If not provided with normal $V_t$, we calculate the normal direction at each point beforehand by linear least squares fitting of a plane over its nearest k neighbors. The algorithm can be described as 4 steps. Firstly selects one point from point clouds as a seed item. Secondly employs k nearest neighbor[] to find its neighbors in the data set. Thirdly includes those neighbors which meet the shape requirements. Lastly repeats procedure for every included neighbor until no further neighbor fulfills the requirements. We ensure that newly formed primitive will not conflict with any existing primitive.\\
% There are 3 requirements for neighbors to be included: accept angle $\alpha$, accept distance $d$ and minimal plane size $n$. Accept angle is the maximum acceptable included angle between plane normal and candidate point normal. Accept distance is the maximum acceptable distance from the point to the estimated plane. Minimal plane size is the minimal number of points to form a plane. If the region ceases growing before reaching minimal size, the whole plane will be discarded and points remain state of undetected. We use Singular Value Decomposition[The singular value decomposition: Its computation and some applications.] to determine plane parameter $S=(A, B, C, D)$ where $Ax+By+Cz+D=0$.\\
% \subsubsection{RANSAC} 
% \label{sec:ransac}
% stands for RANdom SAmple Consensus, a method that iteratively estimates parameters to find the plane with the largest support in the point cloud. Compared with region grow algorithm, RANSAC doesn't require normal estimation, which is more consistent in some sparse scenario like low-resolution point cloud segmentation. We fit 8 planes to each frame of MSR-Action3D[], and the visual effect is illustrated in Fig~\ref{fig:fitting}(b).
% \textbf{TODO: primitive fitting figure of sythia4D HOI4D MSR-Action}\\ 
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=12.3cm]{./figure/primitiveFitting_vis.pdf}
%     \caption{An illustration of Primitive Fitting.  \textbf{a) Region grow on Synthia4D[] and HOI4D[]. } Points with consistent normal direction cluster together. Each primitive region has clear geometric meaning. \textbf{b) RANSAC on MSR-Action3D[]. } Each frame is fitted with 8 planes. Color indicates primitive.}
%     \label{fig:fitting}
% \end{figure}

\subsection{Short-Term Feature Extraction}
\eric{Add an overall introduction for this branch.}

\noindent\textbf{4D Backbone}
We implement our 4D backbone with UNet structure to extract point feature of video. Following the state-of-the-art P4Transformer[], the encoder/decoder is made up of four 4D convolution/decovolution layers. Given clip $\Psi$, the convolution layer can be described as:\\
\begin{equation}
\begin{aligned}
\boldsymbol{f}_{t}^{\prime(x, y, z)}
% =\sum_{\left(\delta_{x}, \delta_{y}, \delta_{z}, \delta_{t}\right) \in G} \zeta\left(\delta_{x}, \delta_{y}, \delta_{z}, \delta_{t}\right) \cdot \boldsymbol{F}_{t+\delta_{t}}^{\left(x+\delta_{x}, y+\delta_{y}, z+\delta_{z}\right)} \\
% &=\sum_{\delta_{t}=-r_{t}}^{r_{t}} \sum_{\left\|\left(\delta_{x}, \delta_{y}, \delta_{z}\right)\right\| \leq r_{s}} \zeta\left(\delta_{x}, \delta_{y}, \delta_{z}, \delta_{t}\right) \cdot \boldsymbol{F}_{t+\delta_{t}}^{\left(x+\delta_{x}, y+\delta_{y}, z+\delta_{z}\right)} \\
&=\sum_{\delta_{t}=-r_{t}}^{r_{t}} \sum_{\left\|\left(\delta_{x}, \delta_{y}, \delta_{z}\right)\right\| \leq r_{s}} 
(\boldsymbol{W_d}\cdot\left(\delta_{x}, \delta_{y}, \delta_{z}, \delta_{t}\right)^T) \odot(\boldsymbol{W_f} \cdot \boldsymbol{f}_{t+\delta_{t}}^{\left(x+\delta_{x}, y+\delta_{y}, z+\delta_{z}\right)})
\end{aligned}
\end{equation}
where $(x, y, z)\in P_t$ and $(\delta_x, \delta_y,\delta_z,\delta_t)$ is spatial-temporal offset of kernel and $\cdot$ is matrix multiplication. $f_t^{(x, y, z)} \in \mathbb{R}^{C\times1}$ is the feature of point at $(x, y, z, t)$, and the temporal aggregation $\sum$ is implemented with sum-pooling and the spatial $\sum$ is max-pooling. $r_s$ and $r_t$ represent temporal and spatial radius. $\boldsymbol{W_d}\cdot\left(\delta_{x}, \delta_{y}, \delta_{z}, \delta_{t}\right)^T$ generates offset weights where $\boldsymbol{W_d} \in \mathbb{R}^{C'\times 4}$ transforms 4D displacements from $\mathbb{R}^{4\times 1}$ to $\mathbb{R}^{C'\times 1}$, and $\boldsymbol{W_f} \in \mathbb{R}^{C'\times C}$ is a projection matrix. $\odot$ is summation. 

\noindent\textbf{Intra-Primitive Transformer}
\label{sec:intra-primitive}
is designed to enhance point features obtained from 4D Convolution[] in a geometry-aware way. Because point clouds are essentially sets embedded in a metric space, self-attention fits naturally for building connections between them. Instead of facilitating information exchange globally, our intra-primitive transformer adopts local aggregation strategy[] to optimize the point embeddings in a geometry-aware way. As shown in Figure~\ref{fig:dataflow}, point features are clustered in groups according to their primitive labels given in primitive fitting phase. Compared with simply grouping by k-NN search in euclidean space[], primitive-based partition has more underlying geometric meaning such as normal consistency. And it additionally enlarges receptive fields by reaching farther points that belonging to the primitive. 

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{./figure/intra.pdf}
    \caption{\textbf{Left: primitive-based region partition.} Points are divided into primitive regions according to primitive labels. Intra-primitive performs self-attention in one primitive region. \textbf{Right: Intra-primitive transformer block.} Consisting of intra-primitive attention layer, pre-LayerNorm, GELU and residual connection.}
    \label{fig:intra}
    % \vspace{-20pt}
\end{figure}

% if we have more exp results...
Specifically, in the layer $i$, the fused feature $F_{out}^i$ of primitive region $i$ with input embedding set  $F_{in}^{i}$ is computed formally as[]:
\begin{equation}
\begin{array}{cc}
     Q= W_q\cdot F_{in}^{i},  K = W_k\cdot F_{in}^{i},  V=W_v\cdot F_{in}^{i} \\
       F_{out}^{i}=SA( Q,  K,  V) = softmax\left(\frac{ Q^T K}{\sqrt{C^k}}\right)V  \\
    %   F_{out}^{k}=  MLP(LN(SA(LN(F_{in}^{k-1}))+F_{in}^{k-1}))
\end{array}
\end{equation}
where $F_{in}^i \in \mathbb{R}^{1\times L\cdot N'\cdot C^i}$, $ L,N',C^i$ represents clip length, point number and input dimension respectively. $W_q, W_k \in \mathbb{R}^{C^k\times C^i}$, $W_k \in \mathbb{R}^{C^v\times C^i}$ where $C^k$ is the key dimension and $C^v$ is value dimension. $Q, K, V$ are queries, keys and values generated from $F_{in}^{i}$. Attention weights  $softmax\left(\frac{ Q^T K}{\sqrt{C^k}}\right)$ is calculated in the primitive region. Note that in this section, we only relate $N'$ embeddings that belong to the same primitive of the \textbf{same frame}. We implement this by efficiently reshaping input feature from $\mathbb{R}^{1\times L N' C^i}$ to $\mathbb{R}^{L\times  N' C^i}$[] and assume the first dimension as 'batch dimension'.\\
As shown in Figure~\ref{fig:intra}, we build intra-primitive transformer block with layernorm, GELU activation, one attentive layer and a following feedforward layer. Feedforward is implemented with a two-layer MLP(Multilayer perception). % TODO: more detail
The output of $l$ layer intra-primitive transformer $F_{out}^l \in \mathbb{R}^{LC^l\times N'}$ is then aggregated by vector max operator $MAX\{\cdot \}$ to obtain primitive level feature $F_{out} \in \mathbb{R}^{LC^l\times 1}$.
% \subsubsection{Memory Pool}
% \label{sec:memorypool}
% stores mid-term representations of primitive region throughout the video, providing complementary long-term information to aid understanding of the current clip. Representations contained in the pool is at primitive level, making long-term point cloud video understanding feasible. After primitive fitting for each frame, we run a 3D backbone[] to acquire point-wise embeddings, then partitioning each frame into regions based on primitives, as demonstrated in Fig\ref{fig:intra}(Left). To extract primitive level representation, point-wise max pool is deployed in every region of video frames. 
% Formally, $M=\{f_{ij}|i=1,\dots,L;j=1,\dots, K\}$ is memory pool which holds a video of $L$ frames, and each frame includes $K$ primitive regions with region features $f$. 
% memory efficient

\subsection{Long-Term Feature}
\label{sec:architecture}
% In this section, we illustrate the core design of hierarchical primitive transformer.

\subsubsection{Inter-Primitive Transformer}
\label{sec:inter-primitive}
is proposed to adaptively combine primitive-level representations from different primitive regions across the video. As demonstrated in Fig~\ref{fig:pipeline}, two streams of embeddings merge here. Fused by intra-primitive transformer, short-term embeddings are of size $M\times L$, where $M$ is the number of primitive region in single frame and $L$ is the clip length. Long-term embeddings support understanding of short-term clip by increasing frame size $L'$ of memory pool. In this fashion, inter-primitive transformer is capable of learning long-term context when processing the current clip. Formally, the input of inter-primitive transformer is $F_{in}^{inter} = [F_{clip} ||  F_{mem}] \in \mathbb{R}^{BC^lM\times (L'+L)}$ which concatenates clip features $F_{clip}$ and long-term features $F_{mem}$. Note that in the inter-primitive attention layer, spatial-temporal attentive aggregation is performed in $M\times(L'+L)$ primitive regions simultaneously. Identical to intra-primitive shown in Fig~\ref{fig:intra}(Right), inter-primitive transformer block is composed of pre-LayerNorm, inter-primitive attention layer, GELU, feedforward layer and residual connection. 

\subsubsection{Semantic segmentation}
% 1. depict segmentation and recognition
% 2. 4D backbone and 3D backbone
\label{sec:segmentation}
For semantic segmentation, the input is clip $\Psi=\{(P_t, V_t ,F_t)|t=1,\dots,c,\dots, L\}$ and the output is the predicted semantic label $l_c$ of frame $c$. We concatenate embeddings of frame $c$ fused by intra-primitive transformer with point-wise feature of frame $c$. Formally, suppose $f_i$ is features of point $i$ extracted by backbone and $e_j$ is the embedding of primitive region $j$. Define $primitive(i) \in [1, M]$ that maps point $i$ to primitive region $j$, and $M$ is the number of region in frame $c$. The output semantic label of point $i$ can be described as $$l_c^i = \zeta([f_i || e_j])$$ where $j = primitive(i)$. And we implement function $\zeta(\cdot)$ with three MLP layers.

\subsubsection{Action Recognition}
\label{sec:recognition}

% ViViT: A Video Vision Transformer

